Quantum intersection rings

We examine a few problems of enumerative geometry and present their solutions in the framework of deformed (quantum) cohomology rings.

==> toc.tex <==
%auto-ignore
\noindent {1.} {Introduction} \leaderfill{1} \par 
\noindent {2.} {Rational curves in $\relax {\fam 0\tenrm I\kern -.18em P}_2$} \leaderfill{3} \par 
\noindent \quad{2.1.} {Preliminaries} \leaderfill{3} \par 
\noindent \quad{2.2.} {Quantum ring} \leaderfill{9} \par 
\noindent \quad{2.3.} {Sketch of an enumerative proof (according to Kontsevich)} \leaderfill{12} \par 
\noindent \quad{2.4.} {Asymptotics} \leaderfill{13} \par 
\noindent \quad{2.5.} {Flat connection} \leaderfill{18} \par 
\noindent \quad{2.6.} {Higher genera} \leaderfill{23} \par 
\noindent \quad{2.7.} {Characteristic numbers} \leaderfill{24} \par 
\noindent {3.} {Rational manifolds} \leaderfill{26} \par 
\noindent \quad{3.1.} {Projective spaces} \leaderfill{27} \par 
\noindent \quad{3.2.} {Quadric surfaces} \leaderfill{31} \par 
\noindent \quad{3.3.} {Cubic surfaces.} \leaderfill{34} \par 
\noindent \quad{3.4.} {Lines in $\relax {\fam 0\tenrm I\kern -.18em P}_3$.} \leaderfill{41} \par 
\noindent \quad{3.5.} {Flags.} \leaderfill{46} \par 
\noindent {4.} {Comments and questions} \leaderfill{51} \par 
\noindent \quad{4.1.} {Manifolds with rational curves} \leaderfill{52} \par 
\noindent \quad{4.2.} {Parallel with matrix models} \leaderfill{54} \par 
\noindent \quad{4.3.} {Partition function} \leaderfill{56} \par 
\noindent \quad{4.4.} {Higher genus} \leaderfill{57} \par 
\noindent \quad{4.5.} {Miscellany} \leaderfill{58} \par 
\noindent Appendix {A.} {} \leaderfill{59} \par 

